Curse or Redemption? How Data Heterogeneity Affects the Robustness of Federated Learning

Data heterogeneity has been identified as one of the key features in federated learning but often overlooked in the lens of robustness to adversarial attacks. This paper focuses on characterizing and understanding its impact on backdooring attacks in federated learning through comprehensive experiments using synthetic and the LEAF benchmarks. The initial impression driven by our experimental results suggests that data heterogeneity is the dominant factor in the effectiveness of attacks and it may be a redemption for defending against backdooring as it makes the attack less efficient, more challenging to design effective attack strategies, and the attack result also becomes less predictable. However, with further investigations, we found data heterogeneity is more of a curse than a redemption as the attack effectiveness can be significantly boosted by simply adjusting the client-side backdooring timing. More importantly,data heterogeneity may result in overfitting at the local training of benign clients, which can be utilized by attackers to disguise themselves and fool skewed-feature based defenses. In addition, effective attack strategies can be made by adjusting attack data distribution. Finally, we discuss the potential directions of defending the curses brought by data heterogeneity. The results and lessons learned from our extensive experiments and analysis offer new insights for designing robust federated learning methods and systems

==> Rebuttal.tex <==

\section{Rebuttal} %(1.75 pages)}
\label{sec:rebuttal}

We thank reviewers for the valuable comments. We address major comments below and all other comments in revision.

\textbf{1. Threat model assumption.} We would like to clarify that in our threat model, each attacker indeed colludes towards the same goal -- embedding the global trigger pattern in the federated model. As shown in \textit{``DBA''} attack, each attacker is aware of the global trigger pattern but \textit{collaboratively} uses a different trigger pattern (part of the global pattern) for colluded attack, which is shown to be more effective than using global pattern for each attacker. Since DBA is an advanced colluded attack (aka side information being distributed global trigger), we believe our assumption is realistic. 

In FL, data privacy is the top priority, thus data sharing among malicious workers may not be an realistic assumption. It has been shown in works \textit{``DBA'', ``Can You Really Backdoor Federated Learning?'', ``Mitigating Sybils in Federated Learning Poisoning''} that collaborative or distributed attacks generally perform better than single device attacks and thus we believe our attacks are sufficiently powerful. We also demonstrate that we can achieve almost 100\% ASR with a low number of malicious datapoints, demonstrating that this is an effective collaborative attack method.

\textbf{2. Other colluding attack strategies.}
Fig.~\ref{fig:rebuttal1} and~\ref{fig:rebuttal2} (the same results as Fig. 4 in submission) show the results of using colluding attack strategies from \textit{``Can You Really Backdoor FL?''} and \textit{``Detecting Backdoor Attacks on Deep Neural Networks by Activation Clustering''} respectively. These results demonstrate our conclusions are generalizable and the poor ASRs are due to data heterogeneity instead of the attack method of \textit{``DBA''}.
%are consistent with the observations in submission.
%and show the results in Figures~\ref{fig:rebuttal1} and~\ref{fig:rebuttal2} respectively. The original observations still hold for different attack strategies.

%\textbf{R1:}
%\textbf{(1) The threat model described in Section 3 present some aspects that look contradictory: Each attacker is limited to the local training and its own model updates, but at the same time, attackers can collude towards the same goal. In my view, this assumption is rather unrealistic.}


% \textbf{This is a common threat model in current state of the art methods for attacking federated learning systems, such as How To Backdoor Federated Learning, Backdoor attacks and defenses in feature-partitioned collaborative learning, Can You Really Backdoor Federated Learning? to name a few. However, it might bring more clarity if we say "The attacker has the capacity to compromise multiple parties."} 

%\PY{We would like to clarify that in our threat model, each attacker indeed colludes towards the same goal -- embedding the global trigger pattern in the federated model. As shown in "DBA" attack, each attacker is aware of the global trigger pattern but \textit{collaboratively} uses a different trigger pattern (part of the global pattern) for colluded attack, which is shown to be more effective than using global pattern for each attacker. Since DBA is an advanced colluded attack (aka side information being distributed global trigger), we believe the assumption is realistic, as mentioned by the reviewer. Moreover, in federated learning setting, data privacy is the top priority. We do not think data sharing among attackers (malicious workers) is an realistic assumption. It has been shown in works DBA, Can You Really Backdoor Federated Learning? and Mitigating Sybils in Federated Learning Poisoning that collaborative or distributed attacks generally perform better than single device attacks and so we believe our attacks are sufficiently powerful. We also demonstrate that we can achieve almost 100\% ASR with a low number of malicious datapoints, demonstrating that this is an effective collaborative attack method.}
\begin{figure}[h] %this figure will be at the right
%\vspace{-5mm}
\centering
  \begin{subfigure}{.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/rebuttal/femnist_1.png}
    %\vspace{-3mm}
    \caption{Using [38] attacks}
    \label{fig:rebuttal1}
  \end{subfigure}
  \begin{subfigure}{.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/rebuttal/femnist_2.png}
     % \vspace{-3mm}
    \caption{Using [10] attacks}
    \label{fig:rebuttal2}
  \end{subfigure}
  \begin{subfigure}{.19\textwidth}
   \vspace{0.5mm}
    \centering
    \includegraphics[width=\linewidth]{images/rebuttal/femnist_scaled_weights.png}
    \caption{Scaling Weights}
    \label{fig:rebuttal5}
  \end{subfigure}
  \begin{subfigure}{.19\textwidth}
    %\vspace{1mm}
    \centering
    \includegraphics[width=\linewidth]{images/rebuttal/femnist_asr_vs_iidness_def_opt.png}
      %\vspace{-3mm}
    \caption{Acc vs. HI}
    \label{fig:rebuttal_4}
  \end{subfigure}
  \begin{subfigure}{.19\textwidth}
    \centering
    %\vspace{2.5mm}
    \includegraphics[width=\linewidth]{images/rebuttal/femnist_3.png}
    \caption{Gaussian Sampling}
    \label{fig:rebuttal3}
  \end{subfigure}
  %\vspace{-2mm}
  \caption{Clarification Results. }%\FY{add legend to d. Maybe also make the font size consistent across figures.}}
  %\vspace{-3mm}
\end{figure}

% \Ali{Do u intend to say unrealistic in last sentence?}
% \PY{No. I want to say data sharing in FL, as proposed by the attacker, is unrealistic.}

% If the attackers collude towards the same objective, it is reasonable to assume that the attackers may have access to some side information or share datasets to craft more powerful attacks. 

% \PY{[I think we can merge this one with previous question.]}
% \Ali{+1}

%\textbf{For example, the attackers may use model poisoning attacks (instead of data poisoning ones) to create more effective backdoor attacks.}
%\vspace{-2mm}
\textbf{3. Model poisoning attack.}
We would like to clarify that when the scaling factor is large, it's effectively doing model replacement (aka model poisoning), see analysis provided in the papers \textit{``DBA''} and \textit{``How to Backdoor Federated Learning''}. We show the scaling factor analysis in Fig.~\ref{fig:rebuttal5}, where high scaled up weights result in strong model poisoning and the results are consistent with not scaled up one (i.e., results in submission). %\FY{Syed is going to add this figure.}
%As pointed out in Threats to Federated Learning: A Survey, data poisoning attacks in Federated Learning are subsumed by model poisoning attacks. (further analysis provided in the papers DBA and How to Backdoor Federated Learning.). 
%\PY{[I recall we have some scaling factor analysis. When the scaling factor is large, it's effectively doing model replacement (aka model poisoning). We can mention the corresponding section.]}
%Model Poisoning attacks generally work by attempting to replace the benign model with a malicious model, which is exactly what data poisoning on local devices hopes to achieve. As pointed out in Threats to Federated Learning: A Survey, data poisoning attacks in Federated Learning are subsumed by model poisoning attacks. (further analysis provided in the papers DBA and How to Backdoor Federated Learning.). We run the same experiments as Fig. 4 using different colluding backdoor attack patterns from Can You Really Backdoor FL? and Detecting Backdoor Attacks on Deep Neural Networks by Activation Clustering and show the results in Figures~\ref{fig:rebuttal1} and~\ref{fig:rebuttal2} respectively. The original observations still hold for different attack strategies.

% \textbf{I think the use of the attack in [41] is not the most appropriate in this scenario: in some cases, the performance look rather poor for experiments where half of the participants are malicious (which is also a not very good scenario to consider).}

% We agree that there can be multiple scenarios of attacks. As such, we perform experiments varying the number of malicious participants and the amount of malicious training data in Section 4.3. We conclude from the observations that the poor ASRs are due to data heterogeneity (which is one of the key observations of our paper) and not because of the attack method of [41], which is backed up by our results in~\ref{fig:rebuttal1} and~\ref{fig:rebuttal2} as well.

%\textbf{(2) Related to the previous comment, although the results in Figure 2 are intuitive, they only apply to the case of the particular attack consider by the authors. In other words, in practical scenarios with colluding attackers (that share datasets or coordinate the malicious model updates), data heterogeneity may not be a barrier to effectively backdoor federated learning algorithms. Thus, the conclusions from the authors may only be applicable on a restricted set of (possibly unrealistic) scenarios.}

%The results reported in Figure 2 considers the scenario of colluding attackers as explained above. This form of backdoor poisoning attack is a very practical threat in Federated Learning currently with a lot of work being done in this area, and our attack model is based upon the standard method of backdooring FL.
% \yuan{Can we be more direct about the response here? Are we saying that our conclusion applies to practical settings? }
% ok - added.
% . To demonstrate the impact of heterogeneity on ASR, we assign the similar data distribution to all the attacking client. Apart from that each malicious client adds the same back door pattern. The updates from the malicious clients selected in a round are aggregated to the global model in the same way as benign participants. We will clarify this in the revision.}  

%\textbf{(3) The results in Section 3 also evidence the same limitations describe before about the threat model and the attack used: it is not reasonable that as the number of attackers increase the performance of the attack decrease.}
\textbf{4. Increasing attackers decreases attack performance and attack budget.}
To make fair comparisons, when we increase the number of attackers, we keep the total number of poisoned data points (i.e., budget) the same. This is also why we use attack budget (to make fair comparison and quantitative analysis on attacks). %We will clarify this in the revision

%\textbf{On the other side, given the threat model described by the authors, I do not understand why they consider the attacker’s budget. If the attacker is in control of the entire training set, there are not restrictions to manipulate the data or the parameters of the model. Of course, by doing this, in some cases the attack could have a negative impact on the performance of the model on benign examples. }
% \textbf{5. Attack budget.}
% The attack budget is not meant to limit the threat model but to quantify the scalability of attackers in terms of both number of data points and number of attackers. In other words, we keep one parameter constant and vary the other, which is why we say attack budget. We will change this to total number of attacker datapoints for clarity.

%\textbf{(4) Related to the previous point, the authors only report the attack success rate, but they have overlooked the performance of the algorithms for different data heterogeneity settings. These results can provide interesting insights related to the relation between attack effectiveness and the overall’s model performance.}
\textbf{5. Attack success rate vs. performance.}
Fig.~\ref{fig:rebuttal_4} shows the results. 
With higher heterogeneity, we observe overall lower performance, which is consistent with the findings of \textit{``Federated Learning with Non-IID data''} and \textit{``TiFL''}.
%and is a common observation, shown in Figure~\ref{fig:rebuttal_4}. We found no interesting relationships between model performance and attack success rate with different heterogeneity settings and so did not discuss it. ASR vs. data heterogeneity is presented in Figure 6.

% \PY{[1. We certainly have ASR vs data heterogeneity analysis; just point the reviewer to the corresponding places in our paper; 2. I think his asking the model performance (test accuracy) v.s. ASR. But I am not sure. ]}
% \yuan{I agree with Pin-Yu that the reviewer might be asking for analysis of test accuracy and ASR.} - So should we add the test accuracy vs. heterogeneity graph? We already have it.

\textbf{6. Comparison with [3].}
%\textbf{(5) In Section 5.1, I think that the authors should discuss how their conclusions compare to those from [3], where aspects related to timing of attacks and persistence of backdoors are considered.}
[3] only focuses on the global attack timing while we investigated both global and local attack timing. The global timing results are consistent with [3] while we additionally provide more insights on local attack timing and local+global attach timing.
%Our conclusions from 5.1 do not contradict [4]s observations. While they demonstrate that persistence can be achieved through their methods, they focus more on the global aspect of attack timing. We show that locally timing our attacks can be very effective while considering the global timing. As such, we build on top of their observations. We will include this in the revision.

%\textbf{(6) Results in Section 5.2 are not revealing anything particularly interesting: the authors are just looking at the last layer and the heterogeneity of the datasets is measured according to the number of target classes contained in the dataset of each participant. Then, it is clear that as the number of classes per participant reduces, the cosine similarity of the parameters in the last layer across clients will reduce. Two questions arise here: does this also happen for the first layers (feature extractors)?}
\textbf{7. Results in Section 5.2 also happen for the first layer?} We did not observe it for the first layer, which is consistent with findings in \textit{``Detecting Backdoor Attacks on Deep Neural Networks by Activation Clustering''}.
%We observe that the feature extraction layers do not differ enough among widely varying data heterogeneousness, which is corroborated by the observations of Detecting Backdoor Attacks on Deep Neural Networks by Activation Clustering. We will discuss this in our revision.


\textbf{8. Other data heterogeneity measure.} We also used Gaussian sampling from the total dataset with the variance denoting the amount of heterogeneity, see Fig.~\ref{fig:rebuttal3}. The results are consistent with the heterogeneity measure using the number of classes, and we adopt the latter in our submission as almost all existing FL papers use it.
%which shows that our observations in the case of sampling without explicit class distribution are the same as well.

%\textbf{What would happen in cases where the data heterogeneity is not related to the number of classes contained in each participant’s dataset but the differences are in the data distribution? For example, in an anomaly detection system (binary classification) where the anomalies provided by each participant may be different.}

%We agree that feature distribution may not be related to the amount of classes. However, current state-of-the-art papers in FL uses this method of generating non-iid data FL with non-iid data. Another method of generating non-iid data is by sampling via a distribution function. We perform such an experiment using Gaussian sampling of the total dataset with the variance denoting the amount of heterogeneity. We present the results for FEMNIST in Figure~\ref{fig:rebuttal3} which shows that our observations in the case of sampling without explicit class distribution are the same as well.

% \textbf{(7) The experiments reported in Section 5.3 look at the class-labels balance across the different clients and, although somewhat related, it does really capture the differences in the underlying data distribution. For example, I can have a binary classification problem where, even if all the clients have the same set of labels, the differences in the data distribution can be huge.}

% We agree that it does not capture 100\% of the differences in the underlying data, which is why even with very low ChiSq values we end up with low ASR in some cases, and we can attribute that to the more complex mechanics of specific data features. However, what we do observe is a weak but nevertheless obvious correlation between class distribution and attack success rates, which we believe sufficiently captures our conclusion that similar dataset distributions yield better ASRs. While class quantity distribution is not a perfect representation of feature distribution, it is a more easily quantifiable and favorable method than random sampling and demonstrates relationships enough to warrant deeper exploration into this phenomenon. We will clarify this in our revision. 

% \textbf{Similarly, as commented before, the conclusions of Section 5.3 heavily depends on the threat model considered and these may not be valid for more realistic attack scenarios.}

% \textbf{(8) Section 6 is very high level and perhaps a bit shallow. The aspects related to defending against backdoors would require a more thorough discussion}

% We will elaborate on the specifics of our proposed defenses. \PY{Are we able to conduct some proof-of-concept defense based on Section 6? We need some numerical evidence to convince the reviewers}

% \textbf{Similarly, the conclusion section is too short and does not capture the contributions of the paper and the future research directions. }

% We will extend our conclusion to be capture our contributions and suggest specific future directions to take.

% \textbf{Other comments:
% - In Section 4.2: how do the authors generate the different malicious data distributions? -}

% We randomly sample these distributions from the total dataset. We will clarify this in the revision

% \textbf{- In Section 6: what do the authors mean by “evading the overfitted weight updates”?}

% It should be "detecting the overfitted weight updates". We will correct this.

\textbf{9. Writing.} We will clarify all the questions and provide more details on defense and conclusion in revision.

% \textbf{R2:}
% \textbf{- Please define distribution index.}

% We will define distribution index more clearly.

\textbf{10. Results on defense.} %\FY{please add the new defense results and descriptions here.} 
We have some proof-of-concept experiments regarding the defenses. 
For \textit{Defense 2}, we implemented a scheduling policy to avoid selecting the same client in nearby rounds (e.g., a client needs to wait at least 20 rounds to be selected again) so that the malicious clients are spreading out further away, which allows FL to forget backdoors easier over time. The results show that with the help of this defend policy, ASR decreases across every heterogeneity level and none of them achieving over 23\% ASR. 
For \textit{Defense 3}, by faking the actual global data distribution, the malicious clients end up building their attack based on a distribution that has a high Chi-Squared value (e.g., about 0.8 in our experiments) compared to the real global distribution. With this defending strategy, the ASRs are much lower -- on average 0.46 (reduced from on average 0.8). 
%The  as explained in Fig. 8 of submission.
%Specifically, the faked global data distribution, when used by the malicious clients yields a ChiSquared value of 0.8 with the real global data. 
%We generate 5 different distributions of malicious clients in such a way, and their ASRs are 0.43, 0.17, 0.56, 0.65 and 0.39.

\textbf{11. Defense using small dataset.} The server trains the global model after one round of aggregation on the small dataset. We keep the dataset small (e.g., 10\% of the total dataset) to reduce cost.

% \textbf{- Defense: please elaborate on how exactly the server will use the small dataset. Will it re-adjust the weights it receives from each party at each round? Isn't it computationally expensive? Does this defense affect the accuracy of the final model?}

% - The server will train the global model after one round of aggregation on the dataset. In order to reduce computational expense and impact on actual training, we keep the dataset small (10\% of the total dataset).

% \texbf{- It seems intuitive that if the data of one party is different, the optimization function for the overall model will try to "average out" these differences as a result not memorizing the backdoor.}
% - Yes, overtime the differences are "averaged out" by the optimization function. However, in order to reduce this effect papers such as DBA and How To Backdoor Federated Learning suggest weight boosting, which is what we use for our attacks as well.

\textbf{12. Test data.} Test data is individually sampled for each client and from each client's entire local dataset.

%\textbf{- Please indicate if test data was used by individual parties and if so how it was distributed.}
%- The test data used by the individual parties are sampled from the total local dataset from that device. It is not distributed across devices in that each device only possesses its own dataset sample.



% \textbf{R3:}
% \textbf{I like the idea of studying the role of data heterogeneity. And indeed this paper
% raises many points that are good to know. However, while I understand that
% all these points are centered around data heterogeneity, the whole paper looks
% like containing a huge pot of different information, including what are potential
% attacks, what are potential defenses, etc. Reading the paper feels like jump around
% among different places.

% With that, I found this paper hard to evaluate (and I am not an expert on the robustness issues of federated learning), and after several passes of reading
% I still feel that the paper lacks some really impressive points that meet the bar
% of a major ML conference. So I decided for now to give this paper a "Weak Reject".
% I could be convinced the other way round however as I learn from other reviewers,
% and from the rebuttal.} 
